Automated Feature-Topic Pairing: Aligning Semantic and Embedding Spaces in Spatial Representation Learning

Automated characterization of spatial data is a kind of critical geographical intelligence. As an emerging technique for characterization, Spatial Representation Learning (SRL) uses deep neural networks (DNNs) to learn non-linear embedded features of spatial data for characterization. However, SRL extracts features by internal layers of DNNs, and thus suffers from lacking semantic labels. Texts of spatial entities, on the other hand, provide semantic understanding of latent feature labels, but is insensible to deep SRL models. How can we teach a SRL model to discover appropriate topic labels in texts and pair learned features with the labels? This paper formulates a new problem: feature-topic pairing, and proposes a novel Particle Swarm Optimization (PSO) based deep learning framework. Specifically, we formulate the feature-topic pairing problem into an automated alignment task between 1) a latent embedding feature space and 2) a textual semantic topic space. We decompose the alignment of the two spaces into: 1) point-wise alignment, denoting the correlation between a topic distribution and an embedding vector; 2) pair-wise alignment, denoting the consistency between a feature-feature similarity matrix and a topic-topic similarity matrix. We design a PSO based solver to simultaneously select an optimal set of topics and learn corresponding features based on the selected topics. We develop a closed loop algorithm to iterate between 1) minimizing losses of representation reconstruction and feature-topic alignment and 2) searching the best topics. Finally, we present extensive experiments to demonstrate the enhanced performance of our method.

==> introduction.tex <==
\vspace{-0.1cm}
\section{Introduction}
%Yanjie
In this paper, we attempt to tackle a long-standing yet critical issue in spatial representation learning (SRL): SRL can learn effective and latent features from geospatial data; these features, however, are  latent without explicit labels. 
In reality, many practical applications require understanding of not just which features are effective, but also what these effective features stand for. 
This issue relates to two tasks: 1) representation learning; 2) label generation for latent features.
Although there has been a rich body of work in SRL~\cite{wang2017region,xu2020multi,wang2018you, wang2018learning, zhang2019unifying, wang2020incremental,chandra2019collective,jean2019tile2vec,zhang2017regions,qian2019spatiotemporal,li2018multi,shan2020geographical}, research in unifying the two tasks is still in its early stage.
In response, we formulate the problem as a task of feature-topic pairing (\textbf{Figure \ref{fig:motivation}}), which is to align a latent embedding feature space, consisting of multiple latent features, and a textual semantic topic space, consisting of multiple topic labels,  by automatically matching the topics with the latent features in SRL.  

\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{graph/Motivation.pdf}
	\vspace{-0.3cm}
	\captionsetup{justification=centering}
	\caption{The motivation of the feature-topic pairing problem: bridging the gap between feature embedding space and topic semantic space in spatial representation learning. }
	\vspace{-0.5cm}
	\label{fig:motivation}
\end{figure}

%Yanjie
Extensive efforts have been made in SRL, including node embedding, autoencoder, random walk, adversarial learning, generative learning based methods with spatial data~\cite{cavallari2017learning,wang2019adversarial,wang2020seqst,qian2019spatiotemporal}. 
Unfortunately, these studies are insufficient to answer what the latent features mean. 
In the era of mobile and Internet of Things, spatial entities usually come with rich textual information ({\it e.g.}, textual description of POIs, review comments), which provides us great opportunities to learn feature representations while identifying the corresponding semantic labels from texts.

%
One of the most intuitive ideas is to extract topics from texts, and, then, pair the topics with the learned latent features during representation learning. 
However, to achieve this goal, three unique challenges (\textbf{Figure \ref{fig:challenges}}) arise:  
(i) How can we construct a textual semantic topic space for spatial entities to support feature-topic pairing?
(ii) How can we quantify the alignment between the explicit topic  space and the latent embedding feature space of spatial entities?
(iii) How can we teach a machine to autonomously select the optimal or the most valuable topic subset to guide feature learning,  match the features with topics, and, moreover, unify feature learning and feature-topic pairing in a closed-loop algorithm?
Next, we outline how we tackle the three challenges.

%Extensive efforts have been made in learning an effective projection from the raw feature space to the target latent representation space with preserving essential properties of spatial entities. For instance, {\it Zhang et al.} uncovered the urban dynamics by a novel cross-modal representation learning framework~\cite{zhang2017regions}, and ~\cite{ding2018geographical} proposed a geographical convolutional neural network to produce location-based embeddings. While promising performances are achieved, the main drawback of the existing literature is that the learned latent representations lack interpretability, which hinders human-readable perception and further decision support. 

%Learning latent vectorized representations is an emerging topic for effective quantification of spatial entities. Effective representation can help us better understand the structures and dynamics of spatial entities, which can further benefit downstream urban computing tasks, such as region planning, forecast travel demand forecasting, traffic congestion prediction, {\it etc.} and ultimately create smart, comfortable and sustainable living environment ~\cite{wang2018ensemble}. 

% literature limitation
%Extensive efforts have been made in learning an effective projection from the raw feature space to the target latent representation space with preserving essential properties of spatial entities. For instance, {\it Zhang et al.} uncovered the urban dynamics by a novel cross-modal representation learning framework~\cite{zhang2017regions}, and ~\cite{ding2018geographical} proposed a geographical convolutional neural network to produce location-based embeddings.  While promising performances are achieved, the main drawback of the existing literature is that the learned latent representations lack interpretability, which hinders human-readable perception and further decision support. 

%Fortunately, spatial entities usually come with rich textual information ({\it e.g.}, textual description of locations, properties, reviews), which provides us with great opportunities to learn interpretable representations by leveraging text semantics.  Intuitively, one of the most natural solutions is to project the text semantic space into the target latent representation space to enhance the interpretability.  However, to achieve the goal, three unique challenges arise:  (i) how can we construct semantic space for spatial entities? (ii) how can we pair the semantic space with the latent representation space of spatial entities? (iii)  how can we reduce the redundancy while paring the two feature spaces?  Next, we outline how we tackle these three challenges as follows.

%Yanjie
\begin{figure}[!t]
	\centering
	\includegraphics[width=\linewidth]{graph/challenge.pdf}
	\vspace{-0.3cm}
	\captionsetup{justification=centering}
	\caption{Key challenges and main tasks of the feature-topic pairing problem. }
	\vspace{-0.5cm}
	\label{fig:challenges}
\end{figure}
First, the semantically-rich texts of spatial entities describe their types, functions, and attribute-related information. 
For instance, on a real estate website, the  texts of a residential community describe crime rates and events, great school ratings,  nearby transportation facilities,  grocery stores, companies, and universities. 
These texts, if properly analyzed, will help to identify which underlying features truly attract residents to pay more to live.  
To discover the semantic labels of  candidate features, we propose to learn a textual semantic topic space: a topic distribution of descriptive texts for each spatial entity.
Specifically, we first extract keywords from the texts of all spatial entities. 
Then, we learn the keyword embedding feature vectors with a pre-trained word embedding model~\cite{hanlp}. 
Finally, we cluster all keyword embeddings by maximizing inter-topic distances and minimizing intra-topic distances to generate topics. In this way, we construct the topic distributions as the semantic space for each entity.
These topics will serve as candidate feature labels, so the deep representation learning model can select the most appropriate topics to pair with embedding features. 

Second, how can we align the topic semantic space with the embedding feature space? 
An intuitive idea is: we can first learn K features for each spatial entities, then select the K best topics that pair with the K features.    
However, in this idea, both feature learning and topic-feature pairing are separated, and, thus, there is no guarantee that the two steps are globally optimized. 
We therefore propose a new strategy: we first let an optimizer to automatically select K topics; the optimizer then guides the representation learner to learn K latent features that optimally align with the K topics. 
The key research question is: how can we quantify the feature-topic alignment? 
To develop a feature-topic alignment measurement, we identify two types of feature-topic alignments: 
(i) point-wise alignment, and (ii) pair-wise alignment.
%what.
First, the point-wise alignment is to describe the correlation between an embedding feature vector and a categorical topic distribution.
In particular, we maximize the correlation so that the distance between the distribution of the embedding vector space and the distribution of the topic semantic vector space can be minimized.
%how and why?
The underlying motivation of point-wise alignment is originated from the fact that:  if a topic density is high in describing a spatial entity, the topic's corresponding feature value is expected to be large to co-vary with the topic density. 
In this way, we align the distribution covariance of the two spaces.  
Second, the pair-wise alignment is to describe the consistency between a feature-feature similarity matrix and a topic-topic similarity matrix. 
In particular, we use the feature-feature similarity graph to describe the topology of the latent embedding feature space, and use the topic-topic similarity graph to describe the topology of the textual semantic topic space. 
If the two spaces are aligned,  the two graphs (represented by matrices) are similar as well. 
By optimizing both alignments, we enforce a better feature-topic pairing. 
%Along this line, we inject the textual semantic into the latent representation space through projection by preserving both the point-wise and pair-wise consistency.

Third, as mentioned above, our framework needs to automatically select the best K-sized topic subset instead of all topics. 
This is because not every learned topic is needed to construct  feature representations in all application scenarios.
%Therefore, the machine needs to decide an optimized topic subset for feature-topic pairing during representation learning. 
Viewing from the feature selection perspective, 
\textit{this is equivalent to the joint task of feature selection and feature label generation. }
We develop a Particle Swarm Optimization (PSO)-based algorithm. 
In this algorithm, we first simultaneously optimize the representation learning loss, point-wise alignment loss, pair-wise alignment loss, and downstream task loss as the feedback for PSO. 
Guided by the feedback, the PSO based algorithm selects a better K-sized topic subset for feature-topic pairing.
In particular, based on the loss function value, PSO iteratively generates topic masks (i.e., 0-1 indicators to select or deselect) to search the optimal topics for space pairing until the learning objective converges.
In this way, the PSO jointly achieves topic selection, feature-topic pairing, and latent feature learning.   

In summary, we propose a new PSO-based framework, named AutoFTP, to unify feature learning,  topic selection, and feature-topic pairing in a single paradigm.
AutoFTP smartly aligns the textual semantic topic space with the latent embedding feature space of spatial entities. 
Our key contributions are: 
1) we movitate and formulate a feature-topic pairing problem; 
2) we propose two measurements (point-wise and pairwise) to measure the alignment between feature space and topic space. 
3) we propose a PSO based method to simtaneously and jointly unify three tasks  representation learning, topic/feature selection, feature-topic pairing  in a single framework;
4) we conduct extensive experiments to validate the effectiveness of the proposed AutoFTP with real world data. 





















